CrIBo: Self-Supervised Learning via Cross-Image Object-Level Bootstrapping

Leveraging nearest neighbor retrieval for self-supervised representation learning has proven beneficial with object-centric images. However, this approach faces limitations when applied to scene-centric datasets, where multiple objects within an image are only implicitly captured in the global representation. Such global bootstrapping can lead to undesirable entanglement of object representations. Furthermore, even object-centric datasets stand to benefit from a finer-grained bootstrapping approach. In response to these challenges, we introduce a novel Cross-Image Object-Level Bootstrapping method tailored to enhance dense visual representation learning. By employing object-level nearest neighbor bootstrapping throughout the training, CrIBo emerges as a notably strong and adequate candidate for in-context learning, leveraging nearest neighbor retrieval at test time. CrIBo shows state-of-the-art performance on the latter task while being highly competitive in more standard downstream segmentation tasks. Our code and pretrained models are publicly available at https://github.com/tileb1/CrIBo.

==> chapters/checklist.tex <==
\section*{Checklist}

The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}
\end{enumerate}

==> chapters/old_method.tex <==










==> chapters/results.tex <==
\section{Results}
\label{sec:results}


==> chapters/todos.tex <==

    



    
    



==> tables/ablation_jump.tex <==
\begin{table}[!ht]
\centering
\caption{
\textbf{TODO}
}
\vspace{0.2cm}
\footnotesize
\resizebox{1\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c c}
 &&& \multicolumn{4}{c}{Pascal VOC} && \multicolumn{4}{c}{ADE20K}  \\
\cmidrule{4-7}  \cmidrule{9-12}
Jump Type & Dataset && 1/128 & 1/64 & 1/8 & 1/1 && 1/128 & 1/64 & 1/8 & 1/1 \\
\midrule
\texttt{no jump} & COCO  && & & & && & & & \\
\texttt{batch jump} & COCO  && & & & && & & & \\
\texttt{queue jump} & COCO  && & & & && & & & \\
\texttt{all jump} & COCO  && & & & && & & & \\
\arrayrulecolor{black!30}\midrule[0.5pt]
\texttt{no jump} & IN1K  && & & & && & & & \\
\texttt{batch jump} & IN1K  && & & & && & & & \\
\texttt{queue jump} & IN1K  && & & & && & & & \\
\texttt{all jump} & IN1K  && & & & && & & & \\
\arrayrulecolor{black}\midrule[0.5pt]
\end{tabular}
\label{table:ablation_jump}
}
\end{table}%

==> tables/finetune_segmenter_segmentation.tex <==
\begin{table}[!ht]
\centering
\caption{
\textbf{Finetuning evaluation with Segmenter.} Backbones pre-trained with different self-supervised learning methods are finetuned using Segmenter \cite{strudel2021segmenter}. We report the mIoU scores achieved on the validation sets of 4 different datasets. Publicly available checkpoints are used when possible, and our reproduced results are indicated with a $\dagger$ symbol.
}
\vspace{0.2cm}
\footnotesize
\resizebox{1\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c}

Method & Backbone & Params & Dataset & Epochs && COCO-Stuff 164K & ADE20K \\
\midrule
\textit{Scene-centric} \\
$\dino^{\dagger}$ \cite{caron2021emerging} & $\vit$-S/16 & 21M & COCO & 300 && 32.2 & 31.7 \\
$\mae$ \cite{he2022masked} & $\vit$-S/16 & 21M & COCO  & 300 && 32.5 & 32.4 \\
$\croc$ \cite{Stegmuller_2023_CVPR} & $\vit$-S/16 & 21M & COCO & 300 && 34.0 & 34.5 \\
\rowcolor{light_cyan} $\mname$ & $\vit$-S/16 & 21M& COCO & 300 && - & -\\
\arrayrulecolor{black!30}\midrule[0.5pt]
\textit{Object-centric} \\
$\dino$ \cite{caron2021emerging} & $\vit$-S/16 & 21M & IN1K & 800 && 34.2 & 35.4 \\
$\croc$ \cite{Stegmuller_2023_CVPR} & $\vit$-S/16 & 21M & IN1K & 300  && 38.4 & 38.1 \\
$\timet$ \cite{salehi2023time} & $\vit$-S/16 & 21M & IN1K+YTVOS  & 800+30 && 35.5 & 36.6 \\
$\dino$ \cite{caron2021emerging} & $\vit$-B/16 & 85M & IN1K & 400 && - & - \\
$\mae$ \cite{he2022masked} & $\vit$-B/16& 85M & IN1K  & ?  && - & -\\
\rowcolor{light_cyan} $\mname$ & $\vit$-S/16 & 21M & IN1K & 300 && - & -    \\
\rowcolor{light_cyan} $\mname$ & $\vit$-B/16 & 85M & IN1K & 400 && - & 38.7 \\
\arrayrulecolor{black}\midrule[0.5pt]
\end{tabular}
\label{table:segmenter_segmentation_old}
}
\end{table}%

==> tables/frozen_linear_segmentation.tex <==
\begin{table}[!ht]
\centering
\caption{
\textbf{Linear segmentation with frozen backbones.} The linear decoder from Segmenter~\cite{strudel2021segmenter} is trained on the frozen spatial features obtained with various self-supervised learning methods. We report the mIoU scores achieved on the validation sets of 4 different datasets. Publicly available checkpoints are used when possible, and our reproduced results are indicated with a $\dagger$ symbol. \TODO{split 4 token}
}
\vspace{0.2cm}
\footnotesize
\resizebox{1\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c c c c c c}
 &  &  &  && \multicolumn{2}{c}{Pascal Context} && \multicolumn{2}{c}{Pascal VOC} && \multicolumn{2}{c}{COCO-Stuff 164K} && \multicolumn{2}{c}{ADE20K} \\
\cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13} \cmidrule{15-16}
Method & Backbone & Epochs & Dataset && $n_{l} = 1$ & $n_{l} = 4$ && $n_{l} = 1$ & $n_{l} = 4$ && $n_{l} = 1$ & $n_{l} = 4$ && $n_{l} = 1$ & $n_{l} = 4$ \\
\midrule
\textit{Scene-centric} \\
$\dino^{\dagger}$ \cite{caron2021emerging} & $\vit$-S/16 & 300 & COCO && 27.3 & 28.9 && 43.9 & 47.4 && 19.9 & 21.6 && 18.9 & 20.3 \\
$\croc$ \cite{Stegmuller_2023_CVPR} & $\vit$-S/16 & 300 & COCO && 30.0 & 32.2 && 51.7 & 54.7 && 22.6 & 25.9 && 20.5 & 24.6  \\
\rowcolor{light_cyan} $\mname$ & $\vit$-S/16 & 300 & COCO && - & - && - & - && - & - && - & -  \\
\arrayrulecolor{black!30}\midrule[0.5pt]
\textit{Object-centric} \\
$\dino$ \cite{caron2021emerging} & $\vit$-S/16 & 800 & IN1K && 32.4 & 41.32 && 49.0 & 69.0 && 24.1 & 33.0 && 23.4 & 31.0 \\
$\croc$ \cite{Stegmuller_2023_CVPR} & $\vit$-S/16 & 300 & IN1K  && 37.7 & 39.9 && 68.1 & 71.4 && 30.2 & 33.4 && 27.6 & 31.3  \\
$\timet$ \cite{salehi2023time} & $\vit$-S/16 & 800+30 & IN1K+YTVOS && 40.6 & 41.9 && 67.9 & 71.9 && 32.0 & 34.5 && 29.9 & 32.3  \\
$\dino$ \cite{caron2021emerging} & $\vit$-B/16 & 400 & IN1K && 38.9 & - && 64.6 & - && - & - && 30.5 & - \\
$\mae$ \cite{he2022masked} & $\vit$-B/16 & ? & IN1K  && - & - && - & - && - & - && - & -  \\
\rowcolor{light_cyan} $\mname$ & $\vit$-S/16 & 300 & IN1K && 40.6 & 41.5 && \textbf{72.3} & \textbf{73.9} && \textbf{33.2} & 34.6 && \textbf{31.3} & \textbf{33.1} \\
\rowcolor{light_cyan} $\mname$ & $\vit$-S/16 & \textcolor{red}{800} & IN1K && 40.7 & 41.6 && 71.9 & 73.4 && - & - && - & -  \\
\rowcolor{light_cyan} $\mname$ & $\vit$-B/16 & \textcolor{red}{400} & IN1K && 42.2 & 42.2 && 73.9 & 74.8 && 35.2 & 35.8 && 34.0 & 34.6  \\
\arrayrulecolor{black}\midrule[0.5pt]
\end{tabular}
\label{table:linear_segmentation}
}
\end{table}%
 %Comparison with other SSL pretrainings on 11 semantic segmentation benchmarks. We report mean IoU on the different validation sets. All methods use ImageNet-1k and ViT-B/16. We use the linear decoder from Segmenter [61] and run evaluation for other methods from their publicly released checkpoints. In the last column, we report the relative improvement over starting from random init. averaged across the 11 datasets. LOCA improves over MAE by +4.3 points.

==> tables/loss_combination_ablation.tex <==
\begin{table*}[h!]
\centering
\caption{\textbf{Ablation study on the individual contribution of each loss.} Run on COCO for 300 epochs and evaluated using dense nearest neighbor retrieval (\cref{table:hummingbird}).}
\footnotesize
\begin{tabular}{c c c c c c}
Config & $\mathcal{L}_{cv}^{g}$ & $\mathcal{L}_{cv}^{o}$ & $\mathcal{L}_{ci}^{o}$ & Pascal VOC & ADE20k \\
 \midrule
1 & \ck & - & - & 31.6 & 12.8 \\
2 & \ck & \ck & - & 47.1 & 18.3\\
\rowcolor{light_cyan} 3 & \ck & \ck & \ck & \textbf{58.1} & \textbf{23.4} \\
\arrayrulecolor{black}\midrule[0.5pt]
\end{tabular}
\label{tab:ablation_loss}
\end{table*}%


==> tables/mask_rcnn.tex <==
\begin{table}[!ht]
\centering
\caption{
\Thomas{
\textbf{Object detection and instance segmentation with Mask R-CNN.} Backbones pre-trained with different self-supervised learning methods are finetuned with a Mask RCNN head \cite{he2017mask}. We report the mean average precision for the predicted bounding boxes ($\text{AP}^{\text{bb}}$) and masks ($\text{AP}^{\text{m}}$) for different IoU thresholds. Publicly available checkpoints are used when possible, and our reproduced results are indicated with a $\dagger$ symbol.
}
}
\vspace{0.2cm}
\footnotesize
\resizebox{1\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c}
 &&&&&& \multicolumn{3}{c}{Object Detection} && \multicolumn{3}{c}{Instance Segmentation}  \\
\cmidrule{7-9} \cmidrule{11-13}
Method & Backbone & Params & Dataset & Epochs && $\text{AP}^{\text{bb}}$ & $\text{AP}^{\text{bb}}_{\text{50}}$ & $\text{AP}^{\text{bb}}_{\text{75}}$ && $\text{AP}^{\text{m}}$ & $\text{AP}^{\text{m}}_{\text{50}}$ & $\text{AP}^{\text{m}}_{\text{75}}$\\
\midrule
\textit{Object-centric} \\
$\dino$ \cite{caron2021emerging} & $\vit$-S/16 & 21M & IN1K & 800 && - & - & - & - & - & - & - \\
$\croc$ \cite{Stegmuller_2023_CVPR} & $\vit$-S/16 & 21M & IN1K & 300 && - & - & - & - & - & - & - \\
$\timet$ \cite{salehi2023time} & $\vit$-S/16 & 21M & IN1K+YTVOS & 800+30 && - & - & - & - & - & - & - \\
\arrayrulecolor{black!30}\midrule[0.5pt]
\textit{Ours} \\
\rowcolor{light_cyan} $\mname$ & $\vit$-S/16 & 21M & IN1K & 800 && - & - & - & - & - & - & - \\
\arrayrulecolor{black}\midrule[0.5pt]
\end{tabular}
\label{table:mask_rcnn}
}
\end{table}%


